The proper motion of HV2112: A T\.ZO candidate in the SMC

The candidate Thorne-\.Zytkow object (T\.ZO), HV2112, is becoming a well-studied if enigmatic object. A key point of its candidacy as a T\.ZO is whether or not it resides in the Small Magellanic Cloud (SMC). HV2112 has detections in a series of photometric catalogues which have resulted in contradictory estimates of its proper motion and, therefore, its membership within the SMC. This letter seeks to resolve the issue of the SMC membership of HV2112 through a reanalysis of extant photometric data. We also demonstrate the difficulties and downfalls inherent in considering a range of catalogue proper motions. We conclude that the proper motion, and associated ancillary radial velocity, positional and photometric properties, are fully consistent with HV2112 being within the SMC and thus it remains a candidate T\.ZO.

==> newtxtext.tex <==
\NeedsTeXFormat{LaTeX2e}

\def\fileversion{1.465}
\def\filedate{2016/01/31}
\ProvidesPackage{newtxtext}[\filedate\space v\fileversion]

\message{`newtxtext' v\fileversion, \filedate\space Text macros taking advantage of TeX-Gyre Termes fonts (msharpe)}
\RequirePackage{fontaxes}% so we can have [bold] italic small caps

\let\orig@footnote=\thefootnote
\let\orig@makefnmark=\@makefnmark
\newdimen\ntx@fs
\RequirePackage{xkeyval,etoolbox}
\renewcommand*{\rmdefault}{ntxtlf} % always TLF for math
\renewcommand*{\familydefault}{\rmdefault}
\def\useosf{\edef\ntx@figurestyle{osf}}
\@onlypreamble\useosf
\def\useproportional{\edef\ntx@figurealign{}}
\@onlypreamble\useproportional

\def\ntx@figurestyle{lf}% default is lining figure style
\def\ntx@figurealign{t}% default is tabular figure alignment
\newif\ifntx@defaultsups
\newif\ifntx@adobesc
\newif\ifntx@scosf
\newif\ifntx@largesc
\newif\ifntx@babel
\ifdefined\bbl@version \ntx@babeltrue\fi
\define@boolkey{ntx}{defaultsups}[true]{%
\csname ntx@defaultsups#1\endcsname}
\define@boolkey{ntx}{largesc}[true]{%
\csname ntx@largesc#1\endcsname}
\define@boolkey{ntx}{adobesc}[true]{%
\csname ntx@adobesc#1\endcsname}
\define@key{ntx}{babel}[true]{%
\csname ntx@babel#1\endcsname}
\newif\ifntx@thrm
\define@key{ntx}{helvratio}[0.9]{\def\ntx@helvratio{#1}}
\define@key{ntx}{scaled}[1.0]{\def\ntx@scaled{s*[#1]}%
\def\ntx@scale{#1}\def\LGCscale{#1}}
\setkeys{ntx}{helvratio} % set this first, at least to default 0.9
\setkeys{ntx}{scaled} % get at least default

\def\ntx@spc{.25em}
\def\ntx@stretch{.2em}
\def\ntx@shrink{.1em}
\define@key{ntx}{spacing}[.25em]{\gdef\ntx@spc{#1}}
\define@key{ntx}{stretch}[.2em]{\gdef\ntx@stretch{#1}}
\define@key{ntx}{shrink}[.1em]{\gdef\ntx@shrink{#1}}


\DeclareOption{lining}{\edef\ntx@figurestyle{lf}}
\DeclareOption{lf}{\edef\ntx@figurestyle{lf}}
\DeclareOption{theoremfont}{\ntx@thrmtrue}
\DeclareOption{oldstyle}{\useosf}
\DeclareOption{osf}{\useosf}
\DeclareOption{tabular}{\edef\ntx@figurealign{t}}
\DeclareOption{p}{\useproportional}
\DeclareOption{proportional}{\useproportional}
%\DeclareOption{sups}{\ntx@defaultsupsfalse}
\DeclareOption{scosf}{\ntx@scosftrue}
\DeclareOption{tighter}{%
\gdef\ntx@spc{.25em}\gdef\ntx@stretch{.15em}\gdef\ntx@shrink{.06em}}
\DeclareOption{looser}{%
\gdef\ntx@spc{.3em}\gdef\ntx@stretch{.2em}\gdef\ntx@shrink{.15em}
}
\ExecuteOptions{lining,tabular}

\DeclareOption*{%
  \begingroup
  \edef\x{\endgroup
    \noexpand\setkeys{ntx}{\CurrentOption}}%
  \x}

\ProcessOptions*
\def\ntx@spacing{%
	\fontdimen2\font=\ntx@spc
	\fontdimen3\font=\ntx@stretch
	\fontdimen4\font=\ntx@shrink
}

\@tempdima=\ntx@scale\p@\@tempdima=\ntx@helvratio\@tempdima%
\edef\qhv@scale{\strip@pt\@tempdima}

\RequirePackage[T1]{fontenc}
\RequirePackage[full]{textcomp}
\DeclareRobustCommand{\sustyle}{%
  \not@math@alphabet\sustyle\relax
  \fontfamily{ntxsups}\selectfont}

\ifntx@scosf %
\DeclareRobustCommand{\textsc}[1]{%
{\fontfamily{ntx\ntx@figurealign osf}\scshape\selectfont #1}%
}\fi% use OsF in small caps

\DeclareRobustCommand{\lfstyle}{%
  \not@math@alphabet\lfstyle\relax
  \fontfamily{ntxlf}\selectfont %
}% to get lf
\DeclareRobustCommand{\tlfstyle}{%
  \not@math@alphabet\tlfstyle\relax
  \fontfamily{ntxtlf}\selectfont %
}% to get tlf
\DeclareRobustCommand{\osfstyle}{%
  \not@math@alphabet\osfstyle\relax
  \fontfamily{ntxosf}\selectfont %
}% to get osf
\DeclareRobustCommand{\tosfstyle}{%
  \not@math@alphabet\tosfstyle\relax
  \fontfamily{ntxtosf}\selectfont %
}% to get tosf
\DeclareRobustCommand{\textlf}[1]{%
  {\lfstyle #1}%
}% to get lf
\DeclareRobustCommand{\texttlf}[1]{%
  {\tlfstyle #1}%
}% to get tlf
\DeclareRobustCommand{\textosf}[1]{%
  {\osfstyle #1}%
}% to get osf
\DeclareRobustCommand{\texttosf}[1]{%
  {\tosfstyle #1}%
}% to get tosf
\DeclareRobustCommand{\textsu}[1]{%
  {\sustyle #1}%
}% to get sup style

\ifntx@thrm
	\ifdefined\newtheoremstyle
	\newtheoremstyle{plain}
	{\topsep}   % ABOVESPACE
    {\topsep}   % BELOWSPACE
    {\slshape}  % BODYFONT--\slshape is defined to be \itshape with upright figures and punctuation
    {}       % INDENT (empty value is the same as 0pt)
    {\bfseries} % HEADFONT--you may want to add \tlfstyle so the number is tab lining, regardless of text figure selection
    {.}         % HEADPUNCT
    {5pt plus 1pt minus 1pt} % HEADSPACE
    {}          % CUSTOM-HEAD-SPEC\newtheorem{thm}{Theorem}[section]
    \fi%
\fi
%\DeclareTextFontCommand{\textsu}{\sustyle}
%\def\@makefnmark{\ifx \thefootnote\orig@footnote \hbox{\sustyle\hspace*{.04em}\@thefnmark}\else\orig@makefnmark\fi}
\ifntx@defaultsups %
\else
  \def\f@@tn@te{footnote}
  \def\@makefnmark{%
    \ifx\@mpfn\f@@tn@te% footnote not in a minipage
      \ifx\thefootnote\orig@footnote%
        \hbox{\sustyle\hspace*{.04em}\@thefnmark\hspace*{.03em}}%
      \else%
        \orig@makefnmark%
      \fi
    \else% footnote in a minipage
%      \ntx@fs=\f@size\p@
%      \ntx@fs=1.05\ntx@fs
%\hbox{{\itshape\sustyle\fontsize{\strip@pt\ntx@fs}{12}\selectfont \@thefnmark\hspace*{.1em}}}%
      \orig@makefnmark%
    \fi}
\fi

%%%%%%%%%%%%%%%%%%%%%%
% Text Serif (Times) %
%%%%%%%%%%%%%%%%%%%%%%

%\renewcommand*{\rmdefault}{ntxr\ntx@style}

%\DeclareSymbolFont{operators}{OT1}{txr}{m}{n}
%\SetSymbolFont{operators}{bold}{OT1}{txr}{bx}{n}
%\def\operator@font{\mathgroup\symoperators}
%
%\DeclareSymbolFont{italic}{OT1}{txr}{m}{it}
%\SetSymbolFont{italic}{bold}{OT1}{txr}{bx}{it}
%
%\DeclareSymbolFontAlphabet{\mathrm}{operators}
%\DeclareMathAlphabet{\mathbf}{OT1}{txr}{bx}{n}
%\DeclareMathAlphabet{\mathit}{OT1}{txr}{m}{it}
%\SetMathAlphabet{\mathit}{bold}{OT1}{txr}{bx}{it}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text Sans Serif (based on Helvetica) %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\renewcommand*{\sfdefault}{qhv}

%\DeclareMathAlphabet{\mathsf}{OT1}{txss}{m}{n}
%\SetMathAlphabet{\mathsf}{bold}{OT1}{txss}{b}{n}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text (Monospaced) Typewriter %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\ttdefault}{ntxtt}

%\DeclareMathAlphabet{\mathtt}{OT1}{txtt}{m}{n}
%\SetMathAlphabet{\mathtt}{bold}{OT1}{txtt}{b}{n}



\def\re@DeclareTextSymbol#1#2#3{%
   \let#1=\undefined
   \DeclareTextSymbol{#1}{#2}{#3}}
   
\def\re@DeclareMathSymbol#1#2#3#4{%
    \let#1=\undefined
    \DeclareMathSymbol{#1}{#2}{#3}{#4}}

\re@DeclareTextSymbol{\L}{OT1}{138}
\re@DeclareTextSymbol{\l}{OT1}{170}
\re@DeclareTextSymbol{\textdollar}{OT1}{36}
\re@DeclareTextSymbol{\textsterling}{OT1}{163}
\re@DeclareMathSymbol{\mathsterling}{\mathord}{operators}{163}

\DeclareTextComposite{\r}{OT1}{A}{197}
\DeclareTextComposite{\r}{OT1}{a}{229}

\re@DeclareTextSymbol{\textcent}{OT1}{162}
\re@DeclareMathSymbol{\mathcent}{\mathord}{operators}{162}

%%% Modification of T1 and LY1 encoding related stuff
%%%

\def\T@n@@nc@d@ng{T1}
\def\T@n@@nc@d@ngM@cr@M@d{%
\DeclareTextCommand{\k}{T1}[1]{{\ooalign{\hidewidth\char12\crcr##1}}}%
}

\def\LY@n@@nc@d@ng{LY1}
\def\LY@n@@nc@d@ngM@cr@M@d{%
\DeclareTextCommand{\k}{LY1}[1]{{\ooalign{\hidewidth\char7\crcr##1}}}%
}

\AtBeginDocument{%
\ifx\encodingdefault\T@n@@nc@d@ng\T@n@@nc@d@ngM@cr@M@d\fi%
\ifx\encodingdefault\LY@n@@nc@d@ng\LY@n@@nc@d@ngM@cr@M@d\fi%
}

\ifntx@babel
	\message{^^JBabel^^J}
\else
	\message{^^JNo Babel^^J}
\fi


\ifntx@babel
    \renewcommand*{\rmdefault}{ntx\ntx@figurealign%
	\ntx@figurestyle}
	\normalfont
\else
    \AtEndPreamble{%
\renewcommand*{\rmdefault}{ntx\ntx@figurealign%
\ntx@figurestyle}
\normalfont}
\fi


\endinput
